Tailor: A Prompt-Based Approach to Attribute-Based Controlled Text Generation

Attribute-based Controlled Text Generation (CTG) refers to generating sentences that satisfy desirable attributes (e.g., emotions and topics). Existing works often utilize fine-tuning or resort to extra attribute classifiers, yet suffer from storage and inference time increases. To address these concerns, we explore attribute-based CTG in a prompt-based manner. In short, the proposed Tailor represents each attribute as a pre-trained continuous vector (i.e., single-attribute prompt) and guides the generation of a fixed PLM switch to a pre-specified attribute. We experimentally find that these prompts can be simply concatenated as a whole to multi-attribute CTG without any re-training, yet raises problems of fluency decrease and position sensitivity. To this end, Tailor provides a multi-attribute prompt mask and a re-indexing position-ids sequence to bridge the gap between the training (one prompt for each task) and testing stage (concatenating more than one prompt). To further enhance such single-attribute prompt combinations, Tailor also introduces a trainable prompt connector, which can be concatenated with any two single-attribute prompts to multi-attribute text generation. Experiments on 11 attribute-specific generation tasks demonstrate strong performances of Tailor on both single-attribute and multi-attribute CTG, with 0.08\% training parameters of a GPT-2.

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/auto_main_multi.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[h]
% \small
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llllllll}
% \toprule
% \multirow{2}{*}{\textbf{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
% \cmidrule(r){3-5} \cmidrule(r){6-7}
% & & All$\uparrow$ & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
% \midrule
% \multicolumn{8}{c}{GPT-2 BASE}   \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \multicolumn{8}{c}{GPT-2 MEDIUM} \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \end{tabular}
% \caption{$\uparrow$ means higher score is better where $\downarrow$ is exactly the opposite. The highest numbers are in \textbf{bold}.}
% \label{}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\small
\centering
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{llc|ccccc}
\toprule
\multirow{2}{*}{\textbf{TP (\%)}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness (\%)}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
\cmidrule(r){3-5} \cmidrule(r){6-7} 
& & Avg $\uparrow$ & Sent $\uparrow$ & Food $\uparrow$ & GRAM $\uparrow$ &PPL $\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
\midrule
% \multicolumn{7}{c}{Full Data Learning}   \\
100.00 &FT   & 69.80 & 74.03 & 65.57 & 0.69  & 46.54 & 0.04 / 0.23 / 0.42  \\
0.60 &Adapter  & 69.10 & 74.10 & 64.10 & 0.77 & 37.89  &  0.03 / 0.21 / 0.42 \\
 0.60 &Adapter (Pseudo) & 81.71 & 89.95 & 73.46 & 0.75 & 45.63 & 0.04 / 0.22 / 0.45  \\
    \cdashline{1-8}[2.5pt/5pt]
0.00 & CONCAT    &  76.20 &  87.88 & 64.51 & 0.63 & 55.02 & 0.05 / 0.33 / 0.68  \\
0.00 &Tailor-C    & 78.82 &  87.54 & 70.10 & 0.63 & 52.76 & 0.05 / 0.32 / 0.68  \\
%  0.08\%&Tailor-W    & 93.35 & 72.38 & 0.68 & 51.29 & 0.05 / 0.34 / 0.70  \\
0.08 &Tailor-W     & 83.98  & 93.27 & 74.68 & 0.68 & 51.41 & 0.05 / 0.33 / 0.69 \\
 0.08 &Tailor-A    & 87.15 & 92.97  & 81.32 & 0.69 & 52.73 & 0.05 / 0.33 / 0.69 \\
\bottomrule
\end{tabular}
\caption{The main results of multi-attribute CTG. Due to space constraints, we average the scores of six combinations (two sentiment attributes $\times$ three topic attributes of food type) as the final results for each method.}
\label{tab:main_multi}
\end{table*}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/auto_main_single.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[h]
% \small
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llllllll}
% \toprule
% \multirow{2}{*}{\textbf{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
% \cmidrule(r){3-5} \cmidrule(r){6-7}
% & & All$\uparrow$ & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
% \midrule
% \multicolumn{8}{c}{GPT-2 BASE}   \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \multicolumn{8}{c}{GPT-2 MEDIUM} \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \end{tabular}
% \caption{$\uparrow$ means higher score is better where $\downarrow$ is exactly the opposite. The highest numbers are in \textbf{bold}.}
% \label{}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llcccc}
\toprule
\multirow{2}{*}{\textbf{TP (\%)}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
\cmidrule(r){4-5} 
& & (\%) $\uparrow$ & GRAM $\uparrow$ &PPL $\downarrow$ & Dist-1/Dist-2/Dist-3 $\uparrow$\\ 
\midrule
% \multicolumn{7}{c}{Full Data Learning}   \\
    % \multirow{10}{*}{30k / Attribute}
    \multirow{2}{*}{100.00} &FT (Food)   & 87.53  & 0.78 & 40.60 &  0.04 / 0.22  / 0.42  \\
    &FT (Sent) & 97.95 & 0.76 & 42.83 & 0.04 / 0.21  / 0.41  \\
    \multirow{2}{*}{0.10} &Adapter (Food) & 74.70 & 0.75 & 43.85 & 0.04 / 0.23 / 0.46 \\
    &Adapter (Sent) & 93.32 & 0.74 & 47.01 & 0.04 / 0.22 / 0.45  \\
    \multirow{2}{*}{0.001}&PPLM (Food) & 60.64 & 0.34 & 105.33 &  0.16 / 0.53 / 0.80 \\
    &PPLM (Sent)  & 69.37 & 0.36 & 75.59 &  0.15 / 0.53 / 0.82  \\
    \multirow{2}{*}{100.00}&GeDi (Food)  & 99.82 & 0.28 & 278.22 &  0.42 / 0.79 / 0.95  \\
    &GeDi (Sent)  & 87.37  &  0.32 &  517.87 &   0.27 / 0.85 / 0.97  \\
    \cdashline{1-6}[2.5pt/5pt]
    \multirow{2}{*}{0.08}&Tailor-S (Food)  & 83.89 & 0.71 & 45.79 & 0.05 / 0.35 / 0.71 \\
    &Tailor-S (Sent)  & 93.80 & 0.71 & 46.20 & 0.06 / 0.35 / 0.70 \\
    % \midrule
% \multicolumn{7}{c}{GPT-2 Medium}   \\
    % \multirow{5}{*}{30k / Attribute}
    % &FT   &   &   &   &   &   \\
    % &Adapter    &   &   &   &   &   \\
    % &PPLM    &   &   &   &   &   \\
    % &GeDi    &   &   &   &   &   \\
    % \cdashline{2-7}[2.5pt/5pt]
    % &Tailor-S    &   &   &   &   &   \\
% \midrule
    % \multicolumn{7}{c}{GPT-2 BASE}   \\
% \multicolumn{7}{c}{Few-Shot Learning}   \\
%     % \multirow{10}{*}{30k / Attribute}
%     \multirow{2}{*}{100.00 \%} &FT (Food Type)   & - & 87.53  & 0.78 & 40.60 &  0.04 / 0.22  / 0.42  \\
%     &FT (Sentiment) & 97.95 & - & 0.76 & 42.83 & 0.04 / 0.21  / 0.41  \\
%     \multirow{2}{*}{0.10 \%} &Adapter (Food Type) & - & 74.70 & 0.75 & 43.85 & 0.04 / 0.23 / 0.46 \\
%     &Adapter (Sentiment) & 93.32 & - & 0.74 & 47.01 & 0.04 / 0.22 / 0.45  \\
%     \multirow{2}{*}{0.001 \%}&PPLM (Food Type) & - & 60.64 & 0.34 & 105.33 &  0.16 / 0.53 / 0.80 \\
%     &PPLM (Sentiment)  & 69.37 & - & 0.36 & 75.59 &  0.15 / 0.53 / 0.82  \\
%     \multirow{2}{*}{100\%}&GeDi (Food Type)  &  -  &   &  &  &  / /  \\
%     &GeDi (Sentiment)  &   & -  &   &   &     /   /   \\
%     \cdashline{2-7}[2.5pt/5pt]
%     \multirow{2}{*}{0.08\%}&Tailor-S (Food Type)  & - & 83.89 & 0.71 & 45.79 & 0.05 / 0.35 / 0.71 \\
%     &Tailor-S (Sentiment)  & 93.80 & - & 0.71 & 46.20 & 0.06 / 0.35 / 0.70 \\
        % \midrule
    % \multicolumn{7}{c}{GPT-2 Medium}   \\
    %     \multirow{5}{*}{3k / Attribute}
    %     &FT   &   &   &   &   &   \\
    %     &Adapter    &   &   &   &   &   \\
    %     &PPLM    &   &   &   &   &   \\
    %     &GeDi    &   &   &   &   &   \\
    %     \cdashline{2-7}[2.5pt/5pt]
    %     &Tailor-S    &   &   &   &   &   \\
\bottomrule
\end{tabular}
\caption{The main results of single-attribute CTG. Due to space constraints, Sent and Food denote averaging the evaluation scores of all sentiment attributes and topics of food type, respectively. TP denotes training parameters as the percentage of the fine-tuning model (FT). $\uparrow$ means higher score is better where $\downarrow$ is exactly the opposite.}
\label{tab:main_single}
\end{table*}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/main_attention.tex <==
\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ll|lll}
\toprule
\multirow{2}{*}{\textbf{Method}}& \multicolumn{3}{c}{\textbf{Correctness (\%)}} \\
\cmidrule(r){2-4}
& Avg$\uparrow$ & Sent$\uparrow$ & Food$\uparrow$\\ 
\midrule
Tailor-C & 78.82 & 87.54 & 70.10 \\
- APA Mask & 78.36 & 87.39 & 69.34 \\
- RP & 77.77  & 88.33 & 67.21 \\
- Both & 76.20 & 87.88 & 64.52 \\
% - APA Mask (S-F) & 77.41 & 85.19 & 69.63 \\
% - APA Mask (F-S) & 79.31 & 89.58 & 69.05 \\
% - RP (S-F) & 78.02 & 85.79 & 70.25 \\
% - RP (F-S) & 77.52 & 90.87 & 64.17 \\
% - Both (S-F)  & 76.10 & 87.35 & 64.85\\
% - Both (F-S)  & 76.30 & 88.41 & 64.18\\
\bottomrule
\end{tabular}
\caption{The ablation study on using the APA mask and the RP sequence (RP) of Tailor-C. `-' denotes removing the corresponding module from Tailor-C. Note that, exchanging the concatenating order of prompts would bring different performances, except for Tailor-C. Thus, we average the scores from these two situations of six attributes combinations as the final result.}


% S-F denotes putting the sentiment attribute prompt in first and food topic attribute prompt in later when concatenating them, in contrast to F-S.}
\label{tab:main_attention}
\end{table}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/main_few_shot.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[h]
% \small
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llllllll}
% \toprule
% \multirow{2}{*}{\textbf{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
% \cmidrule(r){3-5} \cmidrule(r){6-7}
% & & All$\uparrow$ & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
% \midrule
% \multicolumn{8}{c}{GPT-2 BASE}   \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \multicolumn{8}{c}{GPT-2 MEDIUM} \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \end{tabular}
% \caption{$\uparrow$ means higher score is better where $\downarrow$ is exactly the opposite. The highest numbers are in \textbf{bold}.}
% \label{}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lllllll}
\toprule
\multirow{2}{*}{\textbf{TP (\%)}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{Correctness (\%)}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
\cmidrule(r){3-4} \cmidrule(r){5-6} 
& & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
\midrule
    \multicolumn{7}{c}{Single-Attribute CTG} \\
    \multirow{2}{*}{100.00 \%} &FT (Food)   &  - &  54.08 & 0.76 & 38.59 & 0.04 / 0.25 / 0.49  \\
    &FT (Sentiment) & 85.28 & -  & 0.74 & 40.11 & 0.04 / 0.23 / 0.46 \\
    \multirow{2}{*}{0.10 \%} &Adapter (Food) & - & 55.79 & 0.75 & 40.67 & 0.04 / 0.25 / 0.48 \\
    &Adapter (Sentiment) & 77.91 & - & 0.73 & 43.49 & 0.04 / 0.24 / 0.47 \\
    \cdashline{2-7}[2.5pt/5pt]
    \multirow{2}{*}{0.08\%}&Tailor-S (Food)  & - & 66.23  & 0.69 & 41.00 & 0.06 / 0.35 / 0.71 \\
    &Tailor-S (Sentiment)  & 89.27 & - & 0.69 & 41.70 & 0.06 / 0.34 / 0.69  \\
\midrule
    \multicolumn{7}{c}{Multi-Attribute CTG} \\
100 \%    &FT   & 73.45 & 47.75 & 0.73 & 46.29 & 0.04 / 0.25 / 0.48 \\
0.58\% &Adapter  & 68.44 & 45.85 & 0.73 & 45.42 & 0.04 / 0.24 / 0.48 \\
 0.58\% &Adapter (Pseudo Label)    & 78.66 & 55.88 & 0.76 & 40.83 & 0.04 / 0.24 / 0.47 \\
    \cdashline{1-7}[2.5pt/5pt]
0.00\% &Tailor-C    & 74.38 & 61.79 & 0.60 & 47.43 & 0.05 / 0.32 / 0.68 \\
 0.08\%&Tailor-W    & 84.18 & 56.46 & 0.64 & 49.10 & 0.05 / 0.32 / 0.68 \\
 0.08\%&Tailor-A    & 83.63 & 59.18 & 0.63 & 47.78 & 0.05 / 0.32 / 0.68 \\
\bottomrule
\end{tabular}
\caption{The main results of few-Shot learning.}
\label{tab:main_few_shot_all}
\end{table*}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/main_few_shot_short.tex <==
\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lll|ll}
\toprule
\multirow{2}{*}{\textbf{TP (\%)}} &\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Correctness (\%)}} \\ 
\cmidrule(r){3-5} 
& & Avg$\uparrow$& Sent$\uparrow$ & Food$\uparrow$\\ 
\midrule
    \multicolumn{5}{c}{Single-Attribute CTG} \\
    \multirow{2}{*}{100.00} &FT & 54.08 &  - &  54.08 \\
    &FT &85.28 & 85.28 & - \\
    \multirow{2}{*}{0.10} &Adapter &55.79 & - & 55.79 \\
    &Adapter & 77.91 & 77.91 & -  \\
    \cdashline{1-5}[2.5pt/5pt]
    \multirow{2}{*}{0.08}&Tailor-S &66.23 & - & 66.23 \\
    &Tailor-S  & 89.27 & 89.27 & - \\
\midrule
    \multicolumn{5}{c}{Multi-Attribute CTG} \\
100.00&FT   & 60.60 & 73.45 & 47.75 \\
0.60 &Adapter  & 57.15 & 68.44 & 45.85 \\
0.60 &Adapter (Pseudo)    & 67.27 & 78.66 & 55.88 \\
    \cdashline{1-5}[2.5pt/5pt]
0.00 & Tailor-C & 68.09 & 74.38 & 61.79 \\
0.08 & Tailor-W & 70.32 & 84.18 & 56.46 \\
0.08 & Tailor-A & 71.41 & 83.63 & 59.18  \\
\bottomrule
\end{tabular}
\caption{The main results of few-shot learning. Note that TP for multi-Attribute CTG means the extra training parameters as the percentage of the fine-tuning model (FT) after single-Attribute CTG. Due to space constraints, we average the scores of six combinations (two sentiment attributes $\times$ three topic attributes of food type) as the final results for each method.}
\label{tab:main_few_shot_short}
\end{table}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/main_length.tex <==
\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llll}
\toprule
\multirow{2}{*}{\textbf{Model}} &\multirow{2}{*}{\textbf{Length}} & \multicolumn{2}{c}{\textbf{Correctness (\%) }} \\ 
\cmidrule(r){3-4}
& & Sentiment$\uparrow$ & Food$\uparrow$\\ 
\midrule
  \multirow{4}{*}{Tailor-S}& 8  & 86.83 & 72.78 \\
  & 64  & 93.63 & 82.26  \\
  & 128  & 93.80  & 83.89 \\
  & 256 & 96.37 & 87.20 \\
\midrule
  \multirow{4}{*}{Tailor-A} &  8  &  86.60 & 70.26  \\
  &  64  & 93.08 & 76.89 \\
  &  128   & 92.97 & 81.32 \\
  &  256  & 93.86 & 77.82 \\
\bottomrule
\end{tabular}
\caption{The results on multi-attribute CTG of using Tailor-A with different lengths.}
\label{tab:main_length}
\end{table}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/main_sensitivity.tex <==
% \begin{table}[h]
% \small
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{lllll}
% \toprule
% \multirow{2}{*}{\textbf{Method}}& \multirow{2}{*}{\textbf{Combination}} & \multicolumn{2}{c}{\textbf{Correctness (\%)}} \\
% \cmidrule(r){3-4}
% & & Sent$\uparrow$ & Food$\uparrow$\\ 
% \midrule
% \multirow{2}{*}{CONCAT} & NE-AM & 76.93 & 59.87 \\
% & AM-NE & 80.07 & 56.47 \\
% \cdashline{1-4}[2.5pt/5pt]
% \multirow{1}{*}{Tailor-C} &NE-AM / AM-NE & 79.07 & 60.73 \\
% % \multirow{1}{*}{Tailor-A} &PO-ME / ME-PO & 97.87 & 87.13 \\
% \bottomrule
% \end{tabular}
% \caption{The results on multi-attribute CTG of generating sentences satisfying negative
% sentiment (NE) and topic of American food (AM). NE-AM denotes putting the positive attribute prompt in first and American food attribute prompt in later when concatenating them, in contrast to AM-NE.}
% \label{tab:main_sensitivity}
% \end{table}


\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lll|lll}
\toprule
\multirow{2}{*}{\textbf{Method}}& \multirow{2}{*}{\textbf{Combination}} & \multicolumn{3}{c}{\textbf{Correctness (\%)}} \\
\cmidrule(r){3-5}
& & Avg$\uparrow$ & Sent$\uparrow$ & Food$\uparrow$\\ 
\midrule
\multirow{2}{*}{CONCAT} & NE-AM & 68.40 & 76.93 & 59.87 \\
& AM-NE & 68.27 & 80.07 & 56.47 \\
\cdashline{1-5}[2.5pt/5pt]
\multirow{2}{*}{Tailor-C} &NE-AM & 69.90 & 79.07 & 60.73 \\
 &AM-NE & 69.90 & 79.07 & 60.73 \\
% \multirow{1}{*}{Tailor-A} &PO-ME / ME-PO & 97.87 & 87.13 \\
\bottomrule
\end{tabular}
\caption{The results on multi-attribute CTG of generating sentences satisfying negative
sentiment (NE) and topic of American food (AM). NE-AM denotes putting the positive attribute prompt in first and American food attribute prompt in later when concatenating them, in contrast to AM-NE.}
\label{tab:main_sensitivity}
\end{table}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/main_unseen.tex <==
\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lll|lll}
\toprule
\multirow{2}{*}{\textbf{Unseen}}& \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Correctness (\%)}} \\ 
\cmidrule(r){3-5}
& &Avg$\uparrow$ & Sent$\uparrow$ & Food$\uparrow$\\ 
\midrule
PO-ME & Tailor-C & 87.54 & 95.60 & 79.47 \\
PO-ME & Tailor-A & 89.89 & 97.07 & 82.70 \\
-& Tailor-A & 91.64 & 97.87 & 85.40 \\
\bottomrule
\end{tabular}
\caption{The results on unseen combination to multi-attribute CTG. PO-ME denotes the attribute combination of positive sentiment and topic of Mexican food. }
\label{tab:main_unseen}
\end{table}

==> [2022][EMNLP] Tailor_ A Prompt-based Approach to Attribute-Based Controlled Text Generation/table/single_attribute_result_30k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
\cmidrule(r){3-5} \cmidrule(r){6-7}
& & All$\uparrow$ & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
    \midrule
    \multicolumn{8}{c}{GPT-2 BASE} \\
    \midrule
    \multicolumn{8}{c}{GPT-2 MEDIUM} \\

\bottomrule
\end{tabular}
\caption{}
\label{}
\end{table*}

    % \multirow{4}{*}{S-NE} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{S-PO} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{F-ME} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{F-AM} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{F-AS} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\

==> table/main_few_shot.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[h]
% \small
% \centering
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{llllllll}
% \toprule
% \multirow{2}{*}{\textbf{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
% \cmidrule(r){3-5} \cmidrule(r){6-7}
% & & All$\uparrow$ & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
% \midrule
% \multicolumn{8}{c}{GPT-2 BASE}   \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \multicolumn{8}{c}{GPT-2 MEDIUM} \\
%     \multirow{5}{*}{S-NE~+~F-ME}
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AM}  
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
%     \midrule
%     \multirow{5}{*}{S-NE~+~F-AS} 
%     &FT   &   &   &   &   &   \\
%     &PPLM    &   &   &   &   &   \\
%     &Prompt-C    &   &   &   &   &   \\
%     \cdashline{2-8}[2.5pt/5pt]
%     &Tailor-A    &   &   &   &   &   \\
%     &Tailor-W    &   &   &   &   &   \\
% \bottomrule
% \end{tabular}
% \caption{$\uparrow$ means higher score is better where $\downarrow$ is exactly the opposite. The highest numbers are in \textbf{bold}.}
% \label{}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lllllll}
\toprule
\multirow{2}{*}{\textbf{TP (\%)}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{Correctness (\%)}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
\cmidrule(r){3-4} \cmidrule(r){5-6} 
& & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
\midrule
    \multicolumn{7}{c}{Single-Attribute CTG} \\
    \multirow{2}{*}{100.00 \%} &FT (Food)   &  - &  54.08 & 0.76 & 38.59 & 0.04 / 0.25 / 0.49  \\
    &FT (Sentiment) & 85.28 & -  & 0.74 & 40.11 & 0.04 / 0.23 / 0.46 \\
    \multirow{2}{*}{0.10 \%} &Adapter (Food) & - & 55.79 & 0.75 & 40.67 & 0.04 / 0.25 / 0.48 \\
    &Adapter (Sentiment) & 77.91 & - & 0.73 & 43.49 & 0.04 / 0.24 / 0.47 \\
    \cdashline{2-7}[2.5pt/5pt]
    \multirow{2}{*}{0.08\%}&Tailor-S (Food)  & - & 66.23  & 0.69 & 41.00 & 0.06 / 0.35 / 0.71 \\
    &Tailor-S (Sentiment)  & 89.27 & - & 0.69 & 41.70 & 0.06 / 0.34 / 0.69  \\
\midrule
    \multicolumn{7}{c}{Multi-Attribute CTG} \\
100 \%    &FT   & 73.45 & 47.75 & 0.73 & 46.29 & 0.04 / 0.25 / 0.48 \\
0.58\% &Adapter  & 68.44 & 45.85 & 0.73 & 45.42 & 0.04 / 0.24 / 0.48 \\
 0.58\% &Adapter (Pseudo Label)    & 78.66 & 55.88 & 0.76 & 40.83 & 0.04 / 0.24 / 0.47 \\
    \cdashline{1-7}[2.5pt/5pt]
0.00\% &Tailor-C    & 74.38 & 61.79 & 0.60 & 47.43 & 0.05 / 0.32 / 0.68 \\
 0.08\%&Tailor-W    & 84.18 & 56.46 & 0.64 & 49.10 & 0.05 / 0.32 / 0.68 \\
 0.08\%&Tailor-A    & 83.63 & 59.18 & 0.63 & 47.78 & 0.05 / 0.32 / 0.68 \\
\bottomrule
\end{tabular}
\caption{The main results of few-Shot learning.}
\label{tab:main_few_shot_all}
\end{table*}

==> table/main_length.tex <==
\begin{table}[h]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llll}
\toprule
\multirow{2}{*}{\textbf{Model}} &\multirow{2}{*}{\textbf{Length}} & \multicolumn{2}{c}{\textbf{Correctness (\%) }} \\ 
\cmidrule(r){3-4}
& & Sentiment$\uparrow$ & Food$\uparrow$\\ 
\midrule
  \multirow{4}{*}{Tailor-S}& 8  & 86.83 & 72.78 \\
  & 64  & 93.63 & 82.26  \\
  & 128  & 93.80  & 83.89 \\
  & 256 & 96.37 & 87.20 \\
\midrule
  \multirow{4}{*}{Tailor-A} &  8  &  86.60 & 70.26  \\
  &  64  & 93.08 & 76.89 \\
  &  128   & 92.97 & 81.32 \\
  &  256  & 93.86 & 77.82 \\
\bottomrule
\end{tabular}
\caption{The results on multi-attribute CTG of using Tailor-A with different lengths.}
\label{tab:main_length}
\end{table}

==> table/single_attribute_result_30k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\small
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llllllll}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Correctness}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{1}{c}{\textbf{Diversity}} \\ 
\cmidrule(r){3-5} \cmidrule(r){6-7}
& & All$\uparrow$ & Sentiment$\uparrow$ & Food$\uparrow$ & Grammar$\uparrow$ &Perplexity$\downarrow$ & Dist-1/Dist-2/Dist-3$\uparrow$\\ 
    \midrule
    \multicolumn{8}{c}{GPT-2 BASE} \\
    \midrule
    \multicolumn{8}{c}{GPT-2 MEDIUM} \\

\bottomrule
\end{tabular}
\caption{}
\label{}
\end{table*}

    % \multirow{4}{*}{S-NE} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{S-PO} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{F-ME} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{F-AM} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
    % \multirow{4}{*}{F-AS} & FT &   &   &   &   &   &   \\
    % & PPLM  &   &   &   &   &   &   \\
    % & CTRL  &   &   &   &   &   &   \\
    % & Prompt-S   &   &   &   &   &   &   \\
